Network Estimation and Packet Delivery Prediction for Control over Wireless Mesh Networks

Much of the current theory of networked control systems uses simple point-to-point communication models as an abstraction of the underlying network. As a result, the controller has very limited information on the network conditions and performs suboptimally. This work models the underlying wireless multihop mesh network as a graph of links with transmission success probabilities, and uses a recursive Bayesian estimator to provide packet delivery predictions to the controller. The predictions are a joint probability distribution on future packet delivery sequences, and thus capture correlations between successive packet deliveries. We look at finite horizon LQG control over a lossy actuation channel and a perfect sensing channel, both without delay, to study how the controller can compensate for predicted network outages.

==> figures/textext_preamble.tex <==
\usepackage{color}
\usepackage[mathscr]{eucal}
\usepackage{bm}

